MmWave for Extended Reality: Open User Mobility Dataset, Characterisation, and Impact on Link Quality

User mobility in extended reality (XR) can have a major impact on millimeter-wave (mmWave) links and may require dedicated mitigation strategies to ensure reliable connections and avoid outage. The available prior art has predominantly focused on XR applications with constrained user mobility and limited impact on mmWave channels. We have performed dedicated experiments to extend the characterisation of relevant future XR use cases featuring a high degree of user mobility. To this end, we have carried out a tailor-made measurement campaign and conducted a characterisation of the collected tracking data, including the approximation of the data using statistical distributions. Moreover, we have provided an interpretation of the possible impact of the recorded mobility on mmWave technology. The dataset is made publicly accessible to provide a testing ground for wireless system design and to enable further XR mobility modelling.

==> figure/dir-com/architecture/architecture2.tex <==
\begin{tikzpicture}[
    % font=\sffamily,
    roundrec/.style={
        rounded corners=0.5cm
    },
]

\def\waveSpacing{0.2}
\def\rectangleHeight{7.5}

\fill[roundrec, black!20] (0,0.04) rectangle ++(5,\rectangleHeight+0.62);
\fill[roundrec, black!5] (0,0) rectangle ++(5,\rectangleHeight);
\fill[black!5] (0,\rectangleHeight) rectangle ++(5,-1);
\node[anchor=south] at (2.5, \rectangleHeight) {\lsstyle{Surroundings}};

\fill[roundrec, kullogo1!80] (5.85,0.04) rectangle ++(3,\rectangleHeight+0.62);
\fill[roundrec, kullogo1!40] (5.85,0) rectangle ++(3,\rectangleHeight);
\fill[kullogo1!40] (5.85,\rectangleHeight) rectangle ++(3,-1);
\fill[roundrec, kullogo1!40] 
(5.85,0) --
(8.85,0) --
(8.85,\rectangleHeight) --
(5.85,\rectangleHeight) --
(5.85,2.5) --
(3.85,2.5) --
(3.85,0) --
(5.85,0)
; 
\node[anchor=south] at (7.35, \rectangleHeight) {Remote\vphantom{g}};


\foreach \i in {0,...,2}{
    \centerarc[black, very thick, line cap=round](1.2,4.9+\waveSpacing*\i)(60:120:0.5cm); % Vertical
    \centerarc[black, very thick, line cap=round](1.6+\waveSpacing*\i,4.8)(-30:30:0.5cm); % Horizontal
}

\node[anchor=south] (user) at (1.2,0) {\includegraphics[width=2cm]{figure/dir-com/architecture/user.pdf}};

\node[anchor=center, rotate=180, xscale=-1] (ap1) at (1.2,6.8) {\includegraphics[width=1.2cm]{figure/dir-com/architecture/access-point-edited.pdf}};

\node[anchor=center, xscale=-1] (ap2) at (3.8,4.8) {\includegraphics[width=1.2cm]{figure/dir-com/architecture/access-point-edited.pdf}};

\node[anchor=south, xscale=-1] (server) at (7.4,4.5) {\includegraphics[width=1.2cm]{figure/dir-com/architecture/server-storage-edited.pdf}};

\node[anchor=south, xscale=-1] (switch11) at (7.4,3.2) {\includegraphics[width=1cm]{figure/dir-com/architecture/switch-edited.pdf}};
\node[anchor=south, xscale=-1] (switch21) at ([xshift=-0.7cm,yshift=-1cm]switch11.south) {\includegraphics[width=1cm]{figure/dir-com/architecture/switch-edited.pdf}};
\node[anchor=south, xscale=-1] (switch22) at ([xshift=0.7cm,yshift=-1cm]switch11.south) {\includegraphics[width=1cm]{figure/dir-com/architecture/switch-edited.pdf}};
\draw[black, very thick, line cap=round] (switch11.north) --++(0,0.35);
\draw[black, very thick, line cap=round] ([xshift=-0.2cm]switch11.south) --++(-130:0.25cm);
\draw[black] ([xshift=+0.2cm]switch11.south) --++(-50:0.25cm);
% \draw[black, very thick] ([xshift=-0.2cm]switch21.south) --++(-130:0.5cm);
% \draw[black] ([xshift=+0.2cm]switch21.south) --++(-50:0.25cm);
% \node at ([xshift=0.4cm,yshift=-0.35cm]switch21.south) {\dots};
\draw[black] ([xshift=-0.2cm]switch22.south) --++(-130:0.25cm);
\draw[black] ([xshift=+0.2cm]switch22.south) --++(-50:0.25cm);
\node at ([xshift=0.04cm,yshift=-0.35cm]switch22.south) {\dots};

\node[anchor=south, xscale=-1] (pc) at (5.425,0.1) {\includegraphics[width=1.2cm]{figure/dir-com/architecture/cpu-tower-edited.pdf}};

% \draw[rounded corners=0.2cm, black, very thick] 
% (2, 7) 
% -- (5.1, 7)
% -- (5.425, 6.675)
% -- (5.425, 4.1)
% -- (5.425, 3.025)
% -- (5.75, 2.7)
% -- (6.0, 2.7);

% \draw[rounded corners=0.2cm, black, very thick] 
% (4.6, 4.6) 
% -- (5.1, 4.6)
% -- (5.425, 4.275)
% -- (5.425, 2.1);
% % -- (5.425, 1.325)
% % -- (5.75, 1.0)
% % -- (6.1, 1.0);

% \draw[rounded corners=0.2cm, black, very thick] 
% (2, 7) 
% -- (5.1, 7)
% -- (5.425, 6.675)
% -- (5.425, 5.035)
% -- (5.1, 4.7)
% -- (4.6, 4.7);

\draw[rounded corners=0.2cm, black, very thick, line cap=round] 
(2, 7.1) 
-- (5.525, 7.1)
-- (5.525, 2.7)
-- (6.0, 2.7);

\draw[rounded corners=0.2cm, black, very thick, line cap=round] 
(2, 6.92) 
-- (5.325, 6.92)
-- (5.325, 4.7);

\draw[rounded corners=0.2cm, black, very thick, line cap=round] 
(5.325, 4.48)
--(5.325, 4.2);

\draw[rounded corners=0.2cm, black, very thick, line cap=round] 
(4.6, 4.6) 
-- (5.525, 4.6)
-- (5.525, 2.7)
-- (6.0, 2.7);

\draw[rounded corners=0.2cm, black, very thick, line cap=round] 
(4.6, 4.42) 
-- (5.325, 4.42)
-- (5.325, 2.00);

% \draw[rounded corners=0.2cm, black, very thick] 
% -- (5.425, 4.275)
% -- (5.425, 3.025)
% -- (5.75, 2.7)
% -- (6.1, 2.7);

\node[align=center, anchor=center] (sertxt) at ([xshift=-1cm,yshift=0.0cm]server.north) {\small Cloud};
\node[align=center, anchor=center] (fogtxt) at ([xshift=1cm,yshift=0.0cm]switch11.north) {\small Fog};
\node[align=center, anchor=center] (pctxt) at ([xshift=-1cm,yshift=-0.2cm]pc.north) {\small Edge};

\node[align=center] (aptxt) at ([xshift=-0.5cm, yshift=0.4cm]ap2.north) {\small Access point (AP)};
\node[align=center] (usrtxt) at ([xshift=1cm, yshift=0.5cm]user.east) {\small Head-mounted\\\small disp. (HMD) user};

\draw[-{angle 60}, thin] (sertxt.south) to[out=-90, in=150]([yshift=0.7cm]server.east);
\draw[-{angle 60}, thin] (fogtxt.south) to[out=-90, in=50]([xshift=0.1cm,yshift=-0.3cm]switch11.west);
\draw[-{angle 60}, thin] (pctxt.south) to[out=-90, in=150]([yshift=0.2cm]pc.east);

\draw[-{angle 60}, thin] ([xshift=-1.1cm]aptxt.north) --++(135:0.5cm);
\draw[-{angle 60}, thin] ([xshift=-0.58cm]aptxt.south) --++(-45:0.5cm);
\draw[-{angle 60}, thin] (usrtxt.north) to[out=90, in=0] ([xshift=-1cm, yshift=0.5cm]usrtxt.north);
    
\end{tikzpicture}


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> table/mobility_characterisation_v01.tex <==
\resizebox{\linewidth}{!}{

% \begin{tabular}{c|cl|cccccc}
\begin{tabular}{c|cl|rrrrrr|lrrrrrr}
    \toprule

    & \multicolumn{2}{c|}{} & \multicolumn{6}{c|}{\textbf{Measured distribution}} & \multicolumn{7}{c}{\textbf{Fitted distribution}}\\
    
    & \textbf{ID} & \textbf{Quantity} & $\bm{\text{P}_{50}}$ & $\bm{\text{P}_{75}}$ & $\bm{\text{P}_{90}}$ & $\bm{\text{P}_{98}}$ & $\bm{\text{P}_{99}}$ & $\bm{\text{P}_{100}}$ & ~Name & Shape & Loc. & Scale & Min & Max & KS \\
    \midrule
    
    \parbox[t]{1mm}{\multirow{15}{*}{\rotatebox[origin=c]{90}{Head}}} 
    &\multirow{3}{*}{A}&\multirow{3}{*}{\makecell[l]{Planar distance (\SI{}{\meter})}} 
    &\cellcolor{hl_gray}\textbf{\color{RoyalPurple}0.3}&\cellcolor{hl_gray}0.5&\cellcolor{hl_gray}0.8&\cellcolor{hl_gray}1.1&\cellcolor{hl_gray}1.2&\cellcolor{hl_gray}2.0&
    % Gamma&\cellcolor{hl_gray}$y(x) \sim \mathcal{G}(2.06,0,0.19)$&\cellcolor{hl_gray}$0 < x \leq 2.0$\\
    \cellcolor{hl_gray}~Gamma&\cellcolor{hl_gray}2.06&\cellcolor{hl_gray}0&\cellcolor{hl_gray}0.19&\cellcolor{hl_gray}0$<$&\cellcolor{hl_gray}2.0&\cellcolor{hl_gray}0.02\\
    
    &&&\cellcolor{wr_gray}\textbf{\color{RoyalPurple}0.4}&\cellcolor{wr_gray}0.6&\cellcolor{wr_gray}0.9&\cellcolor{wr_gray}1.2&\cellcolor{wr_gray}1.4&\cellcolor{wr_gray}2.3&
    \cellcolor{wr_gray}~Gamma&\cellcolor{wr_gray}2.54&\cellcolor{wr_gray}0&\cellcolor{wr_gray}0.19&\cellcolor{wr_gray}0$<$&\cellcolor{wr_gray}2.3&\cellcolor{wr_gray}0.02\\
    
    &&&\cellcolor{pw_gray}\textbf{\color{RoyalPurple}0.3}&\cellcolor{pw_gray}0.5&\cellcolor{pw_gray}0.7&\cellcolor{pw_gray}0.9&\cellcolor{pw_gray}1.0&\cellcolor{pw_gray}1.4&
    \cellcolor{pw_gray}~Gamma&\cellcolor{pw_gray}2.33&\cellcolor{pw_gray}0&\cellcolor{pw_gray}0.15&\cellcolor{pw_gray}0$<$&\cellcolor{pw_gray}1.4&\cellcolor{pw_gray}0.02\\


    \cline{2-15}
    
    &\multirow{3}{*}{B}&\multirow{3}{*}{\makecell[l]{Vertical distance factor\\[0.25em]{\fontsize{7}{6}\selectfont \textit{Complementary percentile}}}} 
    &\cellcolor{hl_gray}1.0&\cellcolor{hl_gray}0.9&\cellcolor{hl_gray}0.9&\cellcolor{hl_gray}0.5&\cellcolor{hl_gray}0.4&\cellcolor{hl_gray}\textbf{\color{RoyalPurple}0.3}&
    \cellcolor{hl_gray}~Skewed~Cauchy&\cellcolor{hl_gray}-0.54&\cellcolor{hl_gray}0.99&\cellcolor{hl_gray}0.02&\cellcolor{hl_gray}0.3&\cellcolor{hl_gray}1.17&\cellcolor{hl_gray}0.04\\
    
    &&&\cellcolor{wr_gray}0.9&\cellcolor{wr_gray}0.9&\cellcolor{wr_gray}0.8&\cellcolor{wr_gray}0.5&\cellcolor{wr_gray}0.3&\cellcolor{wr_gray}\textbf{\color{RoyalPurple}0.2}&
    \cellcolor{wr_gray}~Skewed~Cauchy&\cellcolor{wr_gray}-0.57&\cellcolor{wr_gray}0.98&\cellcolor{wr_gray}0.04&\cellcolor{wr_gray}0.2&\cellcolor{wr_gray}1.12&\cellcolor{wr_gray}0.04\\
    
    &&&\cellcolor{pw_gray}1.0&\cellcolor{pw_gray}0.9&\cellcolor{pw_gray}0.8&\cellcolor{pw_gray}0.5&\cellcolor{pw_gray}0.5&\cellcolor{pw_gray}\textbf{\color{RoyalPurple}0.3}&
    \cellcolor{pw_gray}~Skewed~Cauchy&\cellcolor{pw_gray}-0.76&\cellcolor{pw_gray}1.00&\cellcolor{pw_gray}0.02&\cellcolor{pw_gray}0.3&\cellcolor{pw_gray}1.18&\cellcolor{pw_gray}0.03\\
    

    \cline{2-15}
    
    &\multirow{3}{*}{C}&\multirow{3}{*}{\makecell[l]{Pitch orientation (\SI{}{\degree})}} 
    &\cellcolor{hl_gray}\textbf{\color{RoyalPurple}20}&\cellcolor{hl_gray}36&\cellcolor{hl_gray}50&\cellcolor{hl_gray}70&\cellcolor{hl_gray}75&\cellcolor{hl_gray}90&
    \cellcolor{hl_gray}~Skewed~Normal&\cellcolor{hl_gray}1.98&\cellcolor{hl_gray}2.96&\cellcolor{hl_gray}28.23&\cellcolor{hl_gray}-80&\cellcolor{hl_gray}90&\cellcolor{hl_gray}0.03\\
    
    &&&\cellcolor{wr_gray}\textbf{\color{RoyalPurple}32}&\cellcolor{wr_gray}47&\cellcolor{wr_gray}59&\cellcolor{wr_gray}74&\cellcolor{wr_gray}79&\cellcolor{wr_gray}90&
    \cellcolor{wr_gray}~Skewed~Normal&\cellcolor{wr_gray}-2.96&\cellcolor{wr_gray}59.32&\cellcolor{wr_gray}41.04&\cellcolor{wr_gray}-82&\cellcolor{wr_gray}90&\cellcolor{wr_gray}0.02\\
    
    &&&\cellcolor{pw_gray}3&\cellcolor{pw_gray}8&\cellcolor{pw_gray}16&\cellcolor{pw_gray}33&\cellcolor{pw_gray}44&\cellcolor{pw_gray}90&
    \cellcolor{pw_gray}~Logistic&\cellcolor{pw_gray}/&\cellcolor{pw_gray}2.85&\cellcolor{pw_gray}5.93&\cellcolor{pw_gray}-70&\cellcolor{pw_gray}90&\cellcolor{pw_gray}0.03\\


    \cline{2-15}
    
    &\multirow{3}{*}{D}&\multirow{3}{*}{\makecell[l]{Lateral velocity (\SI{}{\meter\per\second})}} 
    &\cellcolor{hl_gray}0.1&\cellcolor{hl_gray}0.2&\cellcolor{hl_gray}0.3&\cellcolor{hl_gray}0.6&\cellcolor{hl_gray}0.8&\cellcolor{hl_gray}3.2&
    \cellcolor{hl_gray}~Weibull&\cellcolor{hl_gray}0.93&\cellcolor{hl_gray}0&\cellcolor{hl_gray}0.13&\cellcolor{hl_gray}0$<$&\cellcolor{hl_gray}3.2&\cellcolor{hl_gray}0.04\\
    
    &&&\cellcolor{wr_gray}0.1&\cellcolor{wr_gray}0.2&\cellcolor{wr_gray}0.4&\cellcolor{wr_gray}0.7&\cellcolor{wr_gray}0.9&\cellcolor{wr_gray}2.4&
    \cellcolor{wr_gray}~Weibull&\cellcolor{wr_gray}0.80&\cellcolor{wr_gray}0&\cellcolor{wr_gray}0.12&\cellcolor{wr_gray}0$<$&\cellcolor{wr_gray}2.4&\cellcolor{wr_gray}0.03\\
    
    &&&\cellcolor{pw_gray}0.2&\cellcolor{pw_gray}0.5&\cellcolor{pw_gray}0.9&\cellcolor{pw_gray}1.4&\cellcolor{pw_gray}1.6&\cellcolor{pw_gray}3.2&
    \cellcolor{pw_gray}~Weibull&\cellcolor{pw_gray}0.85&\cellcolor{pw_gray}0&\cellcolor{pw_gray}0.29&\cellcolor{pw_gray}0$<$&\cellcolor{pw_gray}3.2&\cellcolor{pw_gray}0.05\\


    \cline{2-15}
    
    &\multirow{3}{*}{E}&\multirow{3}{*}{\makecell[l]{Angular velocity (\SI{}{\degree\per\second})}} 
    &\cellcolor{hl_gray}15&\cellcolor{hl_gray}38&\cellcolor{hl_gray}83&\cellcolor{hl_gray}180&\cellcolor{hl_gray}224&\cellcolor{hl_gray}\textbf{\color{RoyalPurple}646}&
    \cellcolor{hl_gray}~Log-Normal&\cellcolor{hl_gray}1.27&\cellcolor{hl_gray}0&\cellcolor{hl_gray}15.84&\cellcolor{hl_gray}0$<$&\cellcolor{hl_gray}646&\cellcolor{hl_gray}0.01\\
    
    &&&\cellcolor{wr_gray}10&\cellcolor{wr_gray}27&\cellcolor{wr_gray}63&\cellcolor{wr_gray}158&\cellcolor{wr_gray}197&\cellcolor{wr_gray}\textbf{\color{RoyalPurple}550}&
    \cellcolor{wr_gray}~Log-Normal&\cellcolor{wr_gray}1.38&\cellcolor{wr_gray}0&\cellcolor{wr_gray}10.20&\cellcolor{wr_gray}0$<$&\cellcolor{wr_gray}550&\cellcolor{wr_gray}0.01\\
    
    &&&\cellcolor{pw_gray}21&\cellcolor{pw_gray}42&\cellcolor{pw_gray}79&\cellcolor{pw_gray}166&\cellcolor{pw_gray}208&\cellcolor{pw_gray}\textbf{\color{RoyalPurple}549}&
    \cellcolor{pw_gray}~Log-Normal&\cellcolor{pw_gray}1.04&\cellcolor{pw_gray}0&\cellcolor{pw_gray}20.91&\cellcolor{pw_gray}0$<$&\cellcolor{pw_gray}549&\cellcolor{pw_gray}0.01\\

    
    \midrule
    % \hline

    
    \parbox[t]{1mm}{\multirow{12}{*}{\rotatebox[origin=c]{90}{Hands}}} 
    &\multirow{3}{*}{F}&\multirow{3}{*}{\makecell[l]{Planar distance (\SI{}{\meter})}} 
    &\cellcolor{hl_gray}\textbf{\color{RoyalPurple}0.2}&\cellcolor{hl_gray}0.3&\cellcolor{hl_gray}0.4&\cellcolor{hl_gray}0.6&\cellcolor{hl_gray}0.6&\cellcolor{hl_gray}1.0&
    \cellcolor{hl_gray}~Log-Normal&\cellcolor{hl_gray}0.32&\cellcolor{hl_gray}0&\cellcolor{hl_gray}0.33&\cellcolor{hl_gray}0$<$&\cellcolor{hl_gray}1&\cellcolor{hl_gray}0.04\\
    
    &&&\cellcolor{wr_gray}\textbf{\color{RoyalPurple}0.3}&\cellcolor{wr_gray}0.3&\cellcolor{wr_gray}0.4&\cellcolor{wr_gray}0.5&\cellcolor{wr_gray}0.6&\cellcolor{wr_gray}1.0&
    \cellcolor{wr_gray}~Log-Normal&\cellcolor{wr_gray}0.22&\cellcolor{wr_gray}0&\cellcolor{wr_gray}0.48&\cellcolor{wr_gray}0$<$&\cellcolor{wr_gray}1&\cellcolor{wr_gray}0.01\\
    
    &&&\cellcolor{pw_gray}\textbf{\color{RoyalPurple}0.3}&\cellcolor{pw_gray}0.4&\cellcolor{pw_gray}0.5&\cellcolor{pw_gray}0.6&\cellcolor{pw_gray}0.7&\cellcolor{pw_gray}1.0&
    \cellcolor{pw_gray}~Log-Normal&\cellcolor{pw_gray}0.29&\cellcolor{pw_gray}0&\cellcolor{pw_gray}0.44&\cellcolor{pw_gray}0$<$&\cellcolor{pw_gray}1&\cellcolor{pw_gray}0.03\\
    


    \cline{2-15}
    
    &\multirow{3}{*}{G}&\multirow{3}{*}{\makecell[l]{Vertical distance (\SI{}{\meter})}} 
    &\cellcolor{hl_gray}-0.4&\cellcolor{hl_gray}-0.3&\cellcolor{hl_gray}-0.2&\cellcolor{hl_gray}\textbf{\color{RoyalPurple}0.0}&\cellcolor{hl_gray}0.1&\cellcolor{hl_gray}0.6&
    \cellcolor{hl_gray}~Weibull&\cellcolor{hl_gray}3.91&\cellcolor{hl_gray}-1.17&\cellcolor{hl_gray}0.82&\cellcolor{hl_gray}-1.1&\cellcolor{hl_gray}0.6&\cellcolor{hl_gray}0.05\\
    
    &&&\cellcolor{wr_gray}-0.4&\cellcolor{wr_gray}-0.3&\cellcolor{wr_gray}-0.1&\cellcolor{wr_gray}\textbf{\color{RoyalPurple}0.1}&\cellcolor{wr_gray}0.2&\cellcolor{wr_gray}0.6&
    \cellcolor{wr_gray}~Logistic&\cellcolor{wr_gray}/&\cellcolor{wr_gray}-0.42&\cellcolor{wr_gray}0.13&\cellcolor{wr_gray}-1.1&\cellcolor{wr_gray}0.6&\cellcolor{wr_gray}0.01\\ 
    
    &&&\cellcolor{pw_gray}-0.4&\cellcolor{pw_gray}-0.2&\cellcolor{pw_gray}-0.1&\cellcolor{pw_gray}\textbf{\color{RoyalPurple}0.1}&\cellcolor{pw_gray}0.1&\cellcolor{pw_gray}0.6&
    \cellcolor{pw_gray}~Weibull&\cellcolor{pw_gray}4.45&\cellcolor{pw_gray}-1.51&\cellcolor{pw_gray}1.20&\cellcolor{pw_gray}-1.1&\cellcolor{pw_gray}0.6&\cellcolor{pw_gray}0.06\\



    \cline{2-15}
    
    &\multirow{3}{*}{H}&\multirow{3}{*}{\makecell[l]{Above head duration (\SI{}{\second})}} 
    &\cellcolor{hl_gray}0.5&\cellcolor{hl_gray}1.1&\cellcolor{hl_gray}2.2&\cellcolor{hl_gray}5.4&\cellcolor{hl_gray}7.3&\cellcolor{hl_gray}\textbf{\color{RoyalPurple}22.7}&
    \cellcolor{hl_gray}~Weibull&\cellcolor{hl_gray}0.91&\cellcolor{hl_gray}0&\cellcolor{hl_gray}0.94&\cellcolor{hl_gray}0$<$&\cellcolor{hl_gray}22.7&\cellcolor{hl_gray}0.08\\
    
    &&&\cellcolor{wr_gray}1.3&\cellcolor{wr_gray}3.1&\cellcolor{wr_gray}5.8&\cellcolor{wr_gray}12.6&\cellcolor{wr_gray}16.6&\cellcolor{wr_gray}\textbf{\color{RoyalPurple}46.7}&
    \cellcolor{wr_gray}~Weibull&\cellcolor{wr_gray}0.82&\cellcolor{wr_gray}0&\cellcolor{wr_gray}2.14&\cellcolor{wr_gray}0$<$&\cellcolor{wr_gray}46.7&\cellcolor{wr_gray}0.03\\
    
    &&&\cellcolor{pw_gray}0.4&\cellcolor{pw_gray}0.8&\cellcolor{pw_gray}1.2&\cellcolor{pw_gray}2.1&\cellcolor{pw_gray}2.6&\cellcolor{pw_gray}\textbf{\color{RoyalPurple}22.3}&
    \cellcolor{pw_gray}~Weibull&\cellcolor{pw_gray}1.16&\cellcolor{pw_gray}0&\cellcolor{pw_gray}0.62&\cellcolor{pw_gray}0$<$&\cellcolor{pw_gray}22.3&\cellcolor{pw_gray}0.04\\



    \cline{2-15}
    
    &\multirow{3}{*}{I}&\multirow{3}{*}{\makecell[l]{Lateral velocity (\SI{}{\meter\per\second})}} 
    &\cellcolor{hl_gray}0.1&\cellcolor{hl_gray}0.3&\cellcolor{hl_gray}0.6&\cellcolor{hl_gray}1.3&\cellcolor{hl_gray}1.6&\cellcolor{hl_gray}9.7&
    \cellcolor{hl_gray}~Weibull&\cellcolor{hl_gray}0.84&\cellcolor{hl_gray}0&\cellcolor{hl_gray}0.23&\cellcolor{hl_gray}0$<$&\cellcolor{hl_gray}9.7&\cellcolor{hl_gray}0.04\\
    
    &&&\cellcolor{wr_gray}0.1&\cellcolor{wr_gray}0.3&\cellcolor{wr_gray}0.6&\cellcolor{wr_gray}1.2&\cellcolor{wr_gray}1.4&\cellcolor{wr_gray}9.1&
    \cellcolor{wr_gray}~Weibull&\cellcolor{wr_gray}0.80&\cellcolor{wr_gray}0&\cellcolor{wr_gray}0.20&\cellcolor{wr_gray}0$<$&\cellcolor{wr_gray}9.1&\cellcolor{wr_gray}0.05\\
    
    &&&\cellcolor{pw_gray}0.4&\cellcolor{pw_gray}0.9&\cellcolor{pw_gray}1.7&\cellcolor{pw_gray}3.2&\cellcolor{pw_gray}3.9&\cellcolor{pw_gray}9.9&
    \cellcolor{pw_gray}~Weibull&\cellcolor{pw_gray}0.86&\cellcolor{pw_gray}0&\cellcolor{pw_gray}0.63&\cellcolor{pw_gray}0$<$&\cellcolor{pw_gray}9.9&\cellcolor{pw_gray}0.02\\

    
    
    \bottomrule
\end{tabular}
}

